Chain-of-Probe: Examining the Necessity and Accuracy of CoT Step-by-Step

Current research found the issue of Early Answering in large language models (LLMs), where the models already have an answer before generating the Chain-of-Thought (CoT). This phenomenon suggests a potential lack of necessary dependency between the predicted answer and the reasoning process. Consequently, two important questions arise: (1) Is CoT still necessary if the model already has an answer? (2) Can the correctness of the answer serve as valid evidence for the correctness of CoT? To address these questions, we propose a method, namely Chain-of-Probe (CoP), to probe changes in the mind during the model's reasoning. The probing results show that in a significant number of question-answer cases, CoT appears to be unnecessary, and this necessity correlates with the simplicity of the task, defined by reasoning steps required. Furthermore, by analyzing patterns in mind change, we examine the correctness of the model's reasoning. Our validation reveals that many responses, although correct in their final answer, contain errors in their reasoning process. To this end, we propose a strategic approach based on CoP to prioritize answers with correct reasoning among multiple candidates, thereby bolstering the reliability of the model's reasoning.

==> tables/cot_acc.tex <==
% \begin{table*}[t]
% \centering
% % \begin{adjustbox}{max width=\columnwidth}
% \begin{adjustbox}{max width=0.9\textwidth}
% % \setlength\tabcolsep{3pt}
% % \renewcommand{\arraystretch}{1.1}
% \begin{tabular}{lc|ccc|ccc|c}
% \hline
% \multicolumn{1}{c}{\textbf{Model}} & \textbf{TAFCR (\%)} & \textbf{GS (\%)} & \textbf{CoPS@3(\%)} & \textbf{CoPT (\%)} & \textbf{P (\%)} & \textbf{R (\%)} & \textbf{F 1(\%)} & \textbf{\# Samp.} \\ \hline
% \textbf{Vicuna 7b}                 & 26.7             & 49.1             & 55.3           & 67.6              & 84.1            & 67.2            & 74.7             & 4.17              \\
% \textbf{Mistral 7b}                & 22.5             & 63.7             & 70.7           & 76.4              & 89.6            & 69.3            & 78.1             & 3.89              \\
% \textbf{LLaMA-3 8b}                & 21.7             & 67.4             & 70.6           & 78.9              & 91.0            & 70.3            & 79.3             & 3.53              \\
% \textbf{Qwen2 7b}                  & 19.5             & 71.4             & 75.3           & 82.8              & 91.2            & 70.6            & 79.6             & 3.12              \\
% \textbf{LLaMA-2 7b}                & 19.9             & 55.4             & 60.1           & 68.7              & 81.4            & 72.5            & 76.7             & 4.34              \\
% \textbf{LLaMA-2 13b}               & 17.4             & 60.5             & 65.3           & 72.8              & 87.5            & 67.1            & 76.0             & 3.87              \\
% \textbf{LLaMA-2 70b}               & 20.4             & 66.9             & 76.8           & 81.1              & 91.1            & 71.1            & 79.8             & 4.03              \\ \cdashline{1-9}
% \rowcolor[HTML]{EFEFEF}\textbf{Avg.}                      & 21.1             & 62.0             & 67.7           & 75.5              & 88.0            & 69.7            & 77.7             & 3.89              \\ \hline
% \end{tabular}
% \end{adjustbox}
% \caption{Results of reasoning step correctness verification on ARC-Challenge. TA-FCR stands for True Answer with False CoT Ratio. GS, CoPS@3, and CoPT represent the CoT accuracy under the greedy search, 3-time sampling with the CoP score, and CoP Tree resampling settings, respectively. P, R, and F1 represent precision, recall, and F1-score of the prediction of the CoP Tree, respectively. The groundtruth labels are derived from GPT-4. "\# sample" indicates the average sampling times with the decision tree resampling strategy.} 
% \label{tab:cot_acc}
% \end{table*}

\begin{table*}[h]
\centering
% \begin{adjustbox}{max width=\columnwidth}
\begin{adjustbox}{max width=\textwidth}
% \setlength\tabcolsep{3pt}
% \renewcommand{\arraystretch}{1.1}
\begin{tabular}{lc|ccccc|ccc|c}
\hline
\multicolumn{1}{c}{\textbf{Model}} & \textbf{TAFCR (\%)} & \textbf{GS (\%)} & \textbf{CoPS@3 (\%)} & \textbf{L2M (\%)} & \textbf{ToT (\%)} & \textbf{CoPT (\%)} & \textbf{P (\%)} & \textbf{R (\%)} & \textbf{F 1(\%)} & \textbf{\# Samp.} \\ \hline
\textbf{Vicuna 7b}                 & 26.7                & 49.1             & 55.3                 & 50.0              & 48.7              & \textbf{67.6}      & 84.1            & 67.2            & 74.7             & 4.17              \\
\textbf{Mistral 7b}                & 22.5                & 63.7             & 70.7                 & 71.9              & \textbf{78.6}     & 76.4               & 89.6            & 69.3            & 78.1             & 3.89              \\
\textbf{LLaMA-3 8b}                & 21.7                & 67.4             & 70.6                 & 70.7              & \textbf{79.2}     & 78.9               & 91.0            & 70.3            & 79.3             & 3.53              \\
\textbf{Qwen2 7b}                  & 19.5                & 71.4             & 75.3                 & 78.7              & 81.2              & \textbf{82.8}      & 91.2            & 70.6            & 79.6             & 3.12              \\
\textbf{LLaMA-2 7b}                & 19.9                & 55.4             & 60.1                 & 59.1              & 57.3              & \textbf{68.7}      & 81.4            & 72.5            & 76.7             & 4.34              \\
\textbf{LLaMA-2 13b}               & 17.4                & 60.5             & 65.3                 & 68.5              & 66.7              & \textbf{72.8}      & 87.5            & 67.1            & 76.0             & 3.87              \\
\textbf{LLaMA-2 70b}               & 20.4                & 66.9             & 76.8                 & 74.5              & 79.5              & \textbf{81.1}      & 91.1            & 71.1            & 79.8             & 4.03              \\
\rowcolor[HTML]{EFEFEF}\textbf{Avg.}                      & 21.1                & 62.0             & 67.7                 & 67.6              & 70.2              & \textbf{75.5}      & 88.0            & 69.7            & 77.7             & 3.89              \\ \hline
\end{tabular}
\end{adjustbox}
\caption{Results of reasoning step correctness verification on ARC-Challenge. TA-FCR stands for True Answer with False CoT Ratio. GS, CoPS@3, L2M, ToT, and CoPT represent the CoT accuracy under the greedy search, 3-time sampling with the CoP score, Least-to-Most Prompting, Tree-of-Thought, and CoP Tree resampling settings, respectively. P, R, and F1 represent precision, recall, and F1-score of the prediction of the CoP Tree, respectively. 
% The groundtruth labels are derived from GPT-4. 
"\# sample" indicates the average sampling times with the decision tree resampling strategy.} 
\label{tab:cot_acc}
% \vspace{-0.3cm}
\end{table*}


==> tables/cot_score_selection_app.tex <==
\begin{table*}[t]
\centering
\begin{adjustbox}{max width=\textwidth}
% \renewcommand{\arraystretch}{1.1}
\begin{tabular}{llllllllc}
\hline
\multicolumn{1}{c}{\textbf{Acc (\%)}} & \multicolumn{1}{c}{\textbf{Vicuna 7b}} & \multicolumn{1}{c}{\textbf{Mistral 7b}} & \multicolumn{1}{c}{\textbf{LLaMA-3 8b}} & \multicolumn{1}{c}{\textbf{Qwen2 7b}} & \multicolumn{1}{c}{\textbf{LLaMA-2 7b}} & \multicolumn{1}{c}{\textbf{LLaMA-2 13b}} & \multicolumn{1}{c|}{\textbf{LLaMA-2 70b}} & \textbf{Avg.}             \\ \hline
\rowcolor[HTML]{EFEFEF}\multicolumn{9}{c}{\textbf{\textit{MMLU}}}                                                                                                                                                                                                                                                                                                                                      \\
\textbf{GS}                           & 52.5                                   & 62.7                                    & 67.2                                    & 70.5                                  & 49.7                                    & 55.9                                     & \multicolumn{1}{l|}{69.0}                 & 61.1                     \\
\textbf{Maj@5}                        & 53.6                                   & \textbf{64.5}                           & 69.1                                    & \textbf{73.0}                         & 51.3                                    & 57.7                                     & \multicolumn{1}{l|}{\textbf{70.6}}        & 62.8                     \\
\textbf{CoPS@5}                          & \textbf{54.7 \textcolor{mypink1}{(+1.1)}}                   & 64.4 (-0.1)                             & \textbf{70.2 \textcolor{mypink1}{(+1.1)}}                    & 72.1 (-0.9)                           & \textbf{52.7 \textcolor{mypink1}{(+1.4)}}                    & \textbf{59.0 \textcolor{mypink1}{(+1.3)}}                     & \multicolumn{1}{l|}{69.9 (-0.7)}                 & \textbf{63.3}            \\
\rowcolor[HTML]{EFEFEF}\multicolumn{9}{c}{\textbf{\textit{BBH}}}                                                                                                                                                                                                                                                                                                                                       \\
\textbf{GS}                           & 45.7                                   & 56.5                                    & 71.4                                    & 65.7                                  & 44.1                                    & 48.2                                     & \multicolumn{1}{l|}{63.1}                 & 56.4                     \\
\textbf{Maj@5}                        & 46.9                                   & \textbf{59.2}                           & \textbf{74.0}                           & 68.7                                  & 44.6                                    & 49.6                                     & \multicolumn{1}{l|}{68.5}                 & 58.8                     \\
\textbf{CoPS@5}                          & \textbf{48.5 \textcolor{mypink1}{(+1.6)}}                   & 58.9 (-0.3)                             & 73.4 (-0.6)                             & \textbf{70.1 \textcolor{mypink1}{(+1.4)}}                  & \textbf{45.5 \textcolor{mypink1}{(+0.9)}}                    & \textbf{50.8 \textcolor{mypink1}{(+1.2)}}                     & \multicolumn{1}{l|}{\textbf{69.5} \textcolor{mypink1}{(+1.0)}}        & \textbf{59.5}            \\
\rowcolor[HTML]{EFEFEF}\multicolumn{9}{c}{\textbf{\textit{ARC-Easy}}}                                                                                                                                                                                                                                                                                                                                     \\
\textbf{GS}                           & 81.0                                   & 89.4                                    & 93.5                                    & 94.9                                  & 83.0                                    & 88.4                                     & \multicolumn{1}{l|}{93.4}                 & 89.1                     \\
\textbf{Maj@5}                        & 83.3                                   & 90.9                                    & 94.2                                    & 95.7                                  & 84.5                                    & 88.7                                     & \multicolumn{1}{l|}{94.5}                 & 90.3                     \\
\textbf{CoPS@5}                          & \textbf{84.3 \textcolor{mypink1}{(+1.0)}}                   & \textbf{92.2 \textcolor{mypink1}{(+1.3)}}                    & \textbf{95.2 \textcolor{mypink1}{(+1.0)}}                    & \textbf{96.9 \textcolor{mypink1}{(+1.2)}}                  & \textbf{84.8 \textcolor{mypink1}{(+0.3)}}                    & \textbf{89.0 \textcolor{mypink1}{(+0.3)}}                     & \multicolumn{1}{l|}{\textbf{95.8} \textcolor{mypink1}{(+1.3)}}        & \textbf{91.2}            \\
\rowcolor[HTML]{EFEFEF}\multicolumn{9}{c}{\textbf{\textit{ARC-Challenge}}}                                                                                                                                                                                                                                                                                                                                     \\
\textbf{GS}                           & 66.9                                   & 82.2                                    & 86.1                                    & 88.7                                  & 69.2                                    & 73.2                                     & \multicolumn{1}{l|}{84.0}                 & 78.6                     \\
\textbf{Maj@5}                        & 72.2                                   & 82.8                                    & 87.1                                    & 91.0                                  & 71.4                                    & 77.4                                     & \multicolumn{1}{l|}{88.1}                 & 81.4                     \\
\textbf{CoPS@5}                          & \textbf{73.0 \textcolor{mypink1}{(+0.8)}}                   & \textbf{84.1 \textcolor{mypink1}{(+1.3)}}                    & \textbf{87.4 \textcolor{mypink1}{(+0.3)}}                    & \textbf{91.3 \textcolor{mypink1}{(+0.3)}}                  & \textbf{73.3 \textcolor{mypink1}{(+1.9)}}                    & \textbf{78.4 \textcolor{mypink1}{(+1.0)}}                     & \multicolumn{1}{l|}{\textbf{88.4} \textcolor{mypink1}{(+0.3)}}        & \textbf{82.3}            \\ \cdashline{1-9}
\textbf{Avg.}                                  & +1.1                                   & +0.6                                    & +0.5                                    & +0.5                                  & +1.1                                    & +0.9                                     & +0.5                                      & \multicolumn{1}{l}{+0.7} \\ \hline
\end{tabular}
\end{adjustbox}
\caption{The comparison results of CoT selection. GS, Maj@5, and $S$@5 indicate the settings of greedy search, 5-time sampling with majority vote, and 5-time sampling with the CoP score (our method), respectively. The best result is highlighted in \textbf{bold}.The improvements of $S$@5 compared with Maj@5 are listed in parentheses, with the positive improvements marked in \textcolor{mypink1}{red}. The last row shows the average improvement of $S$@5 compared to Maj@5.} 
\label{tab:cot_score_app}
\end{table*}

==> tables/cot_score_selection_backup.tex <==
\begin{table*}[]
\centering
\begin{adjustbox}{max width=\textwidth}
\begin{tabular}{lcccccccc}
\hline
\multicolumn{1}{c}{\textbf{Acc (\%)}} & \textbf{Vicuna 7b} & \textbf{Mistral 7b} & \textbf{LLaMA-3 8b} & \textbf{Qwen2 7b} & \textbf{LLaMA-2 7b} & \textbf{LLaMA-2 13b} & \multicolumn{1}{c|}{\textbf{LLaMA-2 70b}} & \textbf{Avg}  \\ \hline
\rowcolor[HTML]{EFEFEF}\multicolumn{9}{c}{\textit{MMLU}}                                                                                                                                                                                               \\
\textbf{GS}                           &  52.5               & 62.7                & 67.2                & 70.5              & 49.7                & 55.9                 & \multicolumn{1}{c|}{69.0}                 & 61.1          \\
\textbf{Maj@5}                        & 53.6               & \textbf{64.5}       & 69.1                & \textbf{73.0}     & 51.3                & 57.7                 & \multicolumn{1}{c|}{\textbf{70.6}}        & 62.8          \\
\textbf{S@5}                          & \textbf{54.7}      & 64.4                & \textbf{70.2}       & 72.1              & \textbf{52.7}       & \textbf{59.0}        & \multicolumn{1}{c|}{69.9}                 & \textbf{63.3} \\
\rowcolor[HTML]{EFEFEF}\multicolumn{9}{c}{\textit{BBH}}                                                                                                                                                                                                     \\
\textbf{GS}                           & 45.7               & 56.5                & 71.4                & 65.7              & 44.1                & 48.2                 & \multicolumn{1}{c|}{63.1}                 & 56.4          \\
\textbf{Maj@5}                        & 46.9               & \textbf{59.2}       & \textbf{74.0}       & 68.7              & 44.6                & 49.6                 & \multicolumn{1}{c|}{68.5}                 & 58.8          \\
\textbf{S@5}                          & \textbf{48.5}      & 58.9                & 73.4                & \textbf{70.1}     & \textbf{45.5}       & \textbf{50.8}        & \multicolumn{1}{c|}{\textbf{69.5}}        & \textbf{59.5} \\
\rowcolor[HTML]{EFEFEF}\multicolumn{9}{c}{\textit{ARC-e}}                                                                                                                                                                                                    \\
\textbf{GS}                           & 81.0               & 89.4                & 93.5                & 94.9              & 83.0                & 88.4                 & \multicolumn{1}{c|}{93.4}                 & 89.1          \\
\textbf{Maj@5}                        & 83.3               & 90.9                & 94.2                & 95.7              & 84.5                & 88.7                 & \multicolumn{1}{c|}{94.5}                 & 90.3          \\
\textbf{S@5}                          & \textbf{84.3}      & \textbf{92.2}       & \textbf{95.2}       & \textbf{96.9}     & \textbf{84.8}       & \textbf{89.0}        & \multicolumn{1}{c|}{\textbf{95.8}}        & \textbf{91.2} \\
\rowcolor[HTML]{EFEFEF}\multicolumn{9}{c}{\textit{ARC-c}}                                                                                                                                                                                                 \\
\textbf{GS}                           & 66.9               & 82.2                & 86.1                & 88.7              & 69.2                & 73.2                 & \multicolumn{1}{c|}{84.0}                 & 78.6          \\
\textbf{Maj@5}                        & 72.2               & 82.8                & 87.1                & 91.0              & 71.4                & 77.4                 & \multicolumn{1}{c|}{88.1}                 & 81.4          \\
\textbf{S@5}                          & \textbf{73.0}      & \textbf{84.1}       & \textbf{87.4}       & \textbf{91.3}     & \textbf{73.3}       & \textbf{78.4}        & \multicolumn{1}{c|}{\textbf{88.4}}        & \textbf{82.3} \\ \hline
\end{tabular}

\end{adjustbox}
\caption{The comparison results of CoT selection. GS, Maj@5, and S@5 indicate the settings of greedy search, 5-time sampling with majority vote, and 5-time sampling with the CoT score (our method), respectively. The best result is highlighted in \textbf{bold}.} 
\label{tab:cot_score_full}
\end{table*}
